The Garden of Forking Paths: Towards Multi-Future Trajectory Prediction

This paper studies the problem of predicting the distribution over multiple possible future paths of people as they move through various visual scenes. We make two main contributions. The first contribution is a new dataset, created in a realistic 3D simulator, which is based on real world trajectory data, and then extrapolated by human annotators to achieve different latent goals. This provides the first benchmark for quantitative evaluation of the models to predict multi-future trajectories. The second contribution is a new model to generate multiple plausible future trajectories, which contains novel designs of using multi-scale location encodings and convolutional RNNs over graphs. We refer to our model as Multiverse. We show that our model achieves the best results on our dataset, as well as on the real-world VIRAT/ActEV dataset (which just contains one possible future).

==> Junwei/abstract.tex <==
\begin{abstract}
 This paper studies the problem of predicting the distribution over multiple possible future paths of people as they move through various visual scenes.
 We make two main contributions.
 The first contribution is a new dataset, created in a realistic 3D simulator,
 which is based on real world trajectory data, and then
 extrapolated by human annotators to achieve different latent goals.
 This provides a benchmark for quantitative evaluation
 of the ability of models to predict multiple plausible futures.
 The second contribution is a new model,
 which combines convolutional RNNs, graph attention networks,
 semantic segmentation, multi-scale location encodings,
 and diverse beam search.
 We show that our model achieves the best results
 on our dataset, as well as on the real-world VIRAT/ActEV dataset
 (which just contains one possible future).
 We will release our data, models and code.
\end{abstract}

==> abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
% 1. summary of the problem
Predicting human behaviors in the near future is critical for many intelligent applications. However the future is uncertain due to the fact that human navigates in the scene with different purpose in mind, different preferences, and other dynamic factors that change in the scene. It is important to predict multiple plausible future to avoid possible dangers in applications such as self-driving cars.
% 2. proposed model
Motivated by this idea, this paper studies the problem of person future path prediction with uncertainty. Our approach jointly models spatial and temporal representations of the scene and utilizes graph attention network to generate sequential predictions. 
% 3. proposed dataset
To effectively evaluate the model's ability to predict multi-future trajectories, we collect a trajectory dataset where human annotators control agents to navigate in 3D simulated scenes with different outcomes based on different latent goals.
% 4. experiments
Experimental results show that our method achieves state-of-the-art performance on a large-scale benchmark and also on our multi-future trajectory dataset. Moreover, our method is able to produce meaningful multiple possibilities of the future in real-world videos.
All code, dataset and model will be released upon acceptance of this paper.
Our dataset provides the first quantitative evaluation of uncertain prediction and our model introduces a simple yet effective architecture for such problem. 
\end{abstract}

==> conclusions.tex <==
\section{Conclusion}
In this paper, we have presented a novel neural network model for multi-future person trajectory prediction.
We utilize a simple yet effective two-stage framework that could take into account of the uncertain future and provide probabilistic inferencing.
We refer to the resulting model as \emph{\fancyname}. 
We propose a new dataset called the Forking Paths dataset annotated by humans to evaluate models ability to predict multi-future trajectories.
We showed the efficacy of our model on both the proposed and recent large-scale video benchmarks on person trajectory prediction.

%Our research goal is to promote human safety in applications such as robotics or autonomous driving. We experiment on the public benchmark ActEV, the primary driver of which is to support public safety and traffic monitoring and management by automatic activity detection in streaming video\footnote{{\footnotesize \url{https://actev.nist.gov/1B-Evaluation}}}. Future research into activity and path prediction may implicate ethical issues around privacy, safety and fairness and ought to be considered carefully before being used in real-world applications. Our method for predicting trajectory and activity has not been tested for different populations of people. As such, it is important to further evaluate these issues before employing the model in situations that may differentially impact people.




==> dataset.tex <==
\section{The Forking Paths Dataset}
\label{sec:dataset}


\begin{figure*}[!t]
	\centering
		\includegraphics[width=1.0\textwidth]{figures/fig3.png}
	\caption{Visualization of the Forking Paths dataset. On the left is an example of the anchor videos and the middle image shows a video sequence of the scene reconstructed from anchor videos. The person in the blue bounding box is the controlled agent and multiple future trajectories annotated by humans are shown by overlaid person frames. The red puddles are the defined destinations. The yellow trajectories are future trajectories of the corresponding uncontrolled agents reconstructed from real videos. The scene semantic segmentation ground truth is shown in the third column and the last column shows all four camera views including the top-down view. Please refer to supplemental material for larger pictures.}  
	\label{fig:dataset}
\end{figure*}

In this section, we describe our human-annotated simulation dataset, called Forking Paths, for multi-future trajectories evaluation. The code, simulation dataset, and models will be released.

\noindent\textbf{Motivation}
% why this dataset, what is it compare to other works
The Forking Paths dataset has been collected with the purpose of providing a benchmark to overcome the shortcoming of trajectory prediction in real-world videos, such as SDD~\cite{robicquet2016learning}, ETH/UCY~\cite{pellegrini2010improving,lerner2007crowds}, KITTI~\cite{geiger2013vision}, nuScenes~\cite{caesar2019nuscenes} and VIRAT/ActEV~\cite{oh2011large}, that is one can only observe one out of many possible future trajectories sampled from the underlying distribution. This is broadly acknowledged in prior works~\cite{makansi2019overcoming,thiede2019analyzing,chai2019multipath,gupta2018social,rhinehart2019precog,rhinehart2018r2p2} but has not yet been addressed. The closet work to ours is a toy simulation used in~\cite{makansi2019overcoming, thiede2019analyzing,chai2019multipath}. Different from ours, it contains only artificial trajectories and zero trajectories from real humans. The simulation is set in a unrealistic 2D space with pedestrians oversimplified as points and vehicles as blocks, where no other scene semantics are provided.
%\lu{I think this toy has no notion of scene semantics right?}\junwei{yes no scene semantics}

%contains no human annotations in a unrealistic 2D space, where pedestrians simplified 
%which a toy dataset is generated but the simulation is far from  with only points as pedestrians and blocks as vehicles 
%To have multiple trajectories generated by humans for each real-world scenario, 

\noindent\textbf{Dataset Overview}
In this work, we use CARLA~\cite{dosovitskiy2017carla}, a photo-realistic open source simulator built on top of the Unreal Engine 4. The Forking Paths dataset is generated by first creating a proxy virtual world anchoring on the real-world video scenes, where the real pedestrian and vehicle trajectories are reconstructed in the virtual world. We choose the real videos from ETH/UCY~\cite{pellegrini2010improving,lerner2007crowds} and VIRAT/ActEV~\cite{oh2011large} for their popularity in trajectory prediction research. Different human annotators first watch the same video clip showing an agent's observable past trajectory (for $t=5$ seconds). After that, they will be asked to control the controlled agent to navigate in the identical simulation scene without bumping into other pedestrians or getting hit by a vehicle.
% why the name,  why it is good for evaluation
As people react differently, forking paths often emerges from the same past trajectory. The forking paths can then be used in evaluate multi-future trajectory prediction.


In summary, we have collected 750 annotated trajectory sequences from 10 annotators. It amounts to 3.2 hours of trajectory sequences, which is comparable to the largest trajectory benchmark VIRAT/ActEV~\cite{2018trecvidawad} (4.5 hours) and 5 times bigger than the common ETH/UCY~\cite{lerner2007crowds,luber2010people} benchmark. For evaluation, we merge the annotated sequences for the same observable trajectories that has on average 5.9 future trajectories for 127 controlled agents.

Thanks to CARLA, our dataset collects ground truth for pixel-precise scene semantic segmentation from 13 classes including sidewalk, road, vehicle, pedestrian, \etc. See Fig.~\ref{f3}. Each trajectory is captured in four camera views (three 45-degree and one top-down view). Data under different weather conditions are also provided but not used in evaluation. %Please refer to the supplemental material for more information about the dataset.

Our dataset has two known limitations. First, there is only one human controlled agent in a scene so there are no interactions between human agents. We found this may not be an issue because our current setting only predicts future trajectory in the next 4.2 seconds and interactions are rare in such a short time. 
Second, any simulation bounds to introduce some artifacts. Note that it is not our intention to get a prefect virtual copy of the real-world scene. Our aim is to have a reasonable simulated scene to solicit reactions from human annotators. 

Despite the above two limitations, Section~\ref{sec:ablation} shows that our model trained on simulation data generalizes reasonably well on real-world videos, and vice versa. The rest of the subsection will summarize the data construction process and please refer to supplementary material for more details.  

%only aim to make the simulated scene close to real-world on scene semantic level, not reconstruct every details. The reconstruction level only needs to be enough for stimulating reactions from human annotators that resemble reality.
%However, we have shown that our model which takes abstract scene semantic segmentation as input can perform well on this dataset as .


%In essence, our dataset re-creates the same real-world dynamic environment that consists of vehicles and crowd of people for different human annotators to ``embodied'' the controlled agent to navigate such that multiple future trajectories originated from the exact same past trajectory are recorded.
%Our dataset consists of 5.9 human-generated future trajectories on average for each controlled agent, compared to previous datasets which only have one per scenario.
%These multiple human-reenacted trajectories under the same past observations are more ideal for evaluation of multi-future trajectory prediction. 
%In this work we only use this dataset for testing.%due to its relatively small size

% what the dataset contains
%Video frames are recorded from multiple viewing angles including 45-degree and top-down view. Other views include body-cam and dash-cam view and each frame comes with an associated depth map which is not used in our experiments. 
%See supplemental material for details of dataset annotations.
% misc


% summary
% Our dataset collection process includes three steps detailed in the following sections:
% (i) re-create both the static and dynamic scene elements anchoring on real-world videos;
% (ii) select or create a pedestrian agent for human to control and define their semantic destinations for each scenario sequence;
% (iii) human annotators ``embodies'' the controlled agent and navigate to the destinations .

%\lu{what's limitation. only one human in the scene; limited iteration among agent; artifacts in the simulation world}. \lu{then say we have transfer experiments to relief your concerns}
%\lu{running out of space; considering slimming the following paragraph  and put them into the supplementary materials. }\junwei{done}
\noindent\textbf{Reconstruction from Real-World Videos.}
% why reconstruct instead of from scratch
Following prior simulation datasets~\cite{gaidon2016virtual,ros2016synthia}, we \textit{semi-automatically} reconstruct seven static scenes and their dynamic elements from the real-world videos in ETH/UCY~\cite{pellegrini2010improving,lerner2007crowds} and VIRAT/ActEV~\cite{oh2011large}.
The static scenes are created manually using Unreal Engine editor and the pedestrians along with vehicles are reconstructed automatically using the original object tracking ground truth. 
We split the videos into 15.2 seconds long sequences to cover the experimental setting of 8 seconds in previous works~\cite{alahi2016social,gupta2018social,liang2019peeking,sadeghian2018sophie,li2019way,zhang2019sr,zhao2019multi} and collect sequences without agent collisions as candidates. We call this dataset the ``anchor'' dataset and it is used in our ablation experiment in Section~\ref{sec:ablation}.
Fig.~\ref{f3} shows a comparison between anchor videos and simulation videos.

%There are four scenes in ETH/UCY and five in VIRAT/ActEV. We exclude two cluttered scenes UNIV and 0002 that will fail simulation reconstruction.
%Hence we manually re-create the 7 remaining static scenes from the existing maps in CARLA~\cite{dosovitskiy2017carla}. 
%For dynamic movement of vehicle and pedestrian, we first convert the ground truth trajectory annotations from the real-world videos to the ground plane using the provided homography matrices.
%We then match the real-world trajectories' origin to correct locations in the re-created scenes. 
%Finally, we run the simulation with the reconstructed agents to automatically create candidate scenario sequences.
%Previous works~\cite{alahi2016social,gupta2018social,liang2019peeking,sadeghian2018sophie,li2019way,zhang2019sr,zhao2019multi} use an experimental setting of 3.2 seconds of observation and prediction for the next 4.8 seconds. We use 4.8 seconds of observation and maximum 10.4 seconds for prediction so that more experimental settings can be performed on our dataset. Hence all the candidate scenario sequences are 15.2 seconds long.

\noindent\textbf{Controlled Agent.}
Given the candidates, we manually select sequences with more than one pedestrian and 
at least one pedestrian could have multiple plausible alternative destinations (they could be going to the car instead of the entrance of a building).
%We edit the trajectories of the selected sequence to remove some unrealistic movements (due to small deviations during the reconstruction process).
We then select one of the pedestrians or create one as the ``controlled agent'' (CA) for each sequence and set meaningful destinations within reach like a car or an entrance of a building.
See Fig.~\ref{f3}. % for an example of the controlled agent and please refer to supplemental material for the sequence editing interface.
For version 1.0 of this dataset, we have selected and modified 127 controlled agents with 343 destinations in seven scenes for human annotation.

\noindent\textbf{Human Annotation.}
Given a sequence from the previous step, annotators are asked to control the CA within this sequence to navigate to the defined destination.
Specifically, each annotation session contains the following steps:
(i) a sequence with one CA and one destination is selected;
(ii) a fixed bird-eye view of the scene with visibility of the marked destination is presented to the annotator, while the simulator loops over the sequence up to the end of the observation period until the annotator press ``READY'';
(iii) the annotator is then spawned in a first-person perspective (or third-person) camera fixed on the CA. The simulator will control the CA up until the end of the observation period and then the annotator can assume controls by using the keyboard to navigate. If the CA collides with other pedestrians or gets hit by a vehicle, or the time limit of 10.4 seconds has reached, the annotator will restart step 3. Otherwise the CA reaches the destination and we will start over for the next sequence from step 1.
We record the controls of the successful annotation session.
Finally, we run the simulator using annotations and record videos from different predefined view points to generate the final dataset.
Please refer to supplemental material for examples of the annotation interface and details on annotation controls.
See Fig.~\ref{f3} for an example of the resulting annotations.



==> experiments.tex <==
%\lu{for 20 model ouput in the Method column use SGAN-PV-20 Ours-20}
% cur act label as future label mAP: 0.40420809803040764
\begin{table*}[]
\centering
\begin{tabular}{l|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Input Types} &  \multicolumn{3}{c|}{minADE\textsubscript{20}} & \multicolumn{3}{c}{minFDE\textsubscript{20}}  \\ \cline{3-8} 
 & & 45-degree         & top-down       & All      & 45-degree         & top-down       & All               \\ \hline \hline
Linear & Traj. &  213.2    & 197.6   & 209.3 & 403.2    & 372.9   & 395.6 \\ 
LSTM  & Traj.              &  204.1   & 185.5   & 199.5 & 386.2    & 357.2   & 379.0  \\ 
Alahi \etal~\cite{alahi2016social}& Traj.         &  198.6    & 179.2   & 193.7 & 378.2    & 347.0   & 370.4  \\ 
Liang \etal~\cite{liang2019peeking}& Traj.+RGB+Seg.   &    185.7 & 166.7 & 180.9 & 357.6 & 326.7 & 349.9   \\ 
Gupta \etal~\cite{gupta2018social}(PV)& Traj.         &  195.4    & 182.4   & 192.1 & 358.7    & 344.9   & 355.3  \\ 
Gupta \etal~\cite{gupta2018social}(V)& Traj.         &  186.1    & 172.8   & 182.8 & 336.9    & 323.3   & 333.5  \\ 
 Ours& Traj.+Seg. & \textbf{170.0}{\scriptsize$\pm0.01$} & \textbf{158.9} & \textbf{167.2} & \textbf{336.2} & \textbf{318.4} & \textbf{331.8}   \\ \hline

\end{tabular}
\caption{Comparison of different methods on the Forking Paths dataset. Lower numbers are better. We repeat each experiment five times with random initialization except Linear. For the input types, ``Traj.'' means the input is ``xy'' coordinates. ``RGB'' means CARLA rendered frames and ``Seg.'' means scene semantic segmentations. All models are trained on VIRAT/ActEV.}
\label{exp-multi}
\end{table*}

\begin{figure*}[!t]
	\centering
		\includegraphics[width=1.0\textwidth]{figures/fig4.png}
	\caption{Qualitative analysis. Column 1-4 are visualization of Social LSTM, Next, Social GAN and ours, respectively. See Section~\ref{sec:exp}.}  
	\label{f4}
\end{figure*}


%----------------------------------------------------------------
\section{Experiments}\label{sec:exp}

This section evaluates our~\emph{\fancyname}~model for multi-future trajectory prediction on the proposed Forking Paths dataset. 
To be consistent with previous works~\cite{liang2019peeking, alahi2016social, gupta2018social,alahi2016social, gupta2018social,sadeghian2018sophie}, we also evaluate our model on the challenging VIRAT/ActEV~\cite{2018trecvidawad,oh2011large} benchmark for single-future path prediction.
%We show that our model outperforms state-of-the-art models on this challenging task on several metrics. 
The dataset, source code, and models will be made available to the public.

\subsection{Evaluation Metrics} 
\noindent\textbf{Single-Future Evaluation.}
%In real-world videos, each trajectory only has one sample of the future. 
In single-future experiment, a model is allowed to have a single most-likely trajectory prediction.
Following prior work~\cite{liang2019peeking,alahi2016social,gupta2018social,sadeghian2018sophie,lee2017desire,hong2019rules,chai2019multipath,rhinehart2019precog}, suppose $\tilde{Y}^i=\tilde{Y}^i_{t=h..h+T}$ is the ground truth trajectory of the $i$-th sample, we use two distance-based error metrics: 
\noindent i) \textit{Average Displacement Error} (ADE): The average Euclidean distance between the ground truth coordinates and the prediction coordinates over all time instants,
\begin{equation}
    \text{ADE} = \frac{ \sum^{N}_{i=1} \sum^{T}_{t=h} \lVert \tilde{Y}^t_i - Y^t_i \rVert_{2}}{N*T_{pred}}
\end{equation}

\noindent ii) \textit{Final Displacement Error} (FDE): The euclidean distance between the predicted points and the ground truth point at the final prediction time instant $T_{pred}$,
\begin{equation}
    \text{FDE} = \frac{ \sum^{N}_{i=1} \lVert \tilde{Y}^{T}_i - Y^{T}_i \rVert_{2}}{N}
\end{equation}

\noindent\textbf{Multi-Future Evaluation.}
For multi-future prediction, we evaluate the models' predicted multi-future trajectories for the same controlled agent (CA). Each CA of the identical historical path has multiple ground-truth future trajectories.
Let $\tilde{Y}_{ij}=\tilde{Y}^{t=h..T}_{ij}$ be the $j$-th true future trajectory for the $i$-th test sample.
Since there is no prior datasets similar to ours, we adapt the commonly used distance-based metrics and define minADE\textsubscript{K}/minFDE\textsubscript{K}. 
%Meanwhile, as our model also outputs distribution over locations, we also measure Negative Log-likelihood (NLL) as in~\cite{chai2019multipath,makansi2019overcoming,kitani2012activity}:

\noindent i) \textit{Minimum Average Displacement Error Given K Predictions} (minADE\textsubscript{K}): similar to the one described in ~\cite{chai2019multipath, rhinehart2018r2p2,rhinehart2019precog, gupta2018social}, 
given K predictions for each sample, we select the closest prediction to compute the error against each ground truth trajectory. The final error is averaged across all time-instants, all ground truth trajectories and all samples. Suppose each sample has $J$ possible ground truth trajectories:
\begin{equation}
    \text{minADE}_K = \frac{  \sum^{N}_{i=1} \sum^{J}_{j=1} \min^j_{Y_{ik}} \sum^{T}_{t=h} \lVert \tilde{Y}^t_{ij} - Y^t_{ik} \rVert_{2}}{N \times T \times J}
\end{equation}

\noindent ii) \textit{Minimum Final Displacement Error Given K Predictions} (minFDE\textsubscript{K}): similar to minADE\textsubscript{K}, but we only consider the predicted points and the ground truth point at the final prediction time instant $T_{pred}$:
\begin{equation}
    \text{minFDE}_K = \frac{  \sum^{N}_{i=1} \sum^{J}_{j=1} \min^j_{Y_{ik}} \lVert \tilde{Y}^{T}_{ij} - Y^{T}_{ik} \rVert_{2}}{N \times J}
\end{equation}


\subsection{Multi-Future Prediction on Forking Paths}\label{sec:exp-multi}

\noindent\textbf{Dataset \& Setups.} 
The proposed Forking Paths dataset in Section~\ref{sec:dataset} is used for multi-future trajectory prediction evaluation. 
%Anchoring on real-world videos, we reconstruct the dynamic scenarios and ask different human annotators to control agents to navigate given the same starting sequences. Multiple future trajectories are thus created based on different human preferences and different intended destinations for the same observations. More details are described in Section~\ref{sec:dataset}.
Following the setting in previous works~\cite{liang2019peeking, alahi2016social, gupta2018social,alahi2016social, gupta2018social,sadeghian2018sophie, makansi2019overcoming}, 
we downsample the videos to 2.5 fps and extract person trajectories using code released in~\cite{liang2019peeking}, and let the models observe 3.2 seconds (8 frames) of the controlled agent before outputting trajectory coordinates in the pixel space. 
Since the length of the ground truth future trajectories are different, each model needs to provide the maximum prediction length at test time and we evaluate the predictions using the actual length of each ground truth trajectory.
We evaluate the models on both 45-degree and top-down camera views.
%We use the pixel values for the trajectory coordinates as it is done in~\cite{yagi2018future, liang2019peeking, lee2017desire, chai2019multipath, li2019way,makansi2019overcoming, bansal2018chauffeurnet,hong2019rules}. 

% TODO(junwei): change the wording of this
\noindent\textbf{Baseline methods.} 
We compare our method with the two simple baselines and three recent methods with released source code. Our baseline includes a recent model for multi-future prediction model and the state-of-the-art model for single-future prediction:
%\textbf{\textit{ConstantV}} is a recent non-parametric method proposed in ~\cite{scholler2019simpler}, which computes a constant velocity for prediction based on the observed trajectories.
\textbf{\textit{Linear}} is a single layer model that predicts the next coordinates using a linear regressor based on the previous input point. 
\textbf{\textit{LSTM}} is a simple LSTM~\cite{hochreiter1997long} encoder-decoder model with coordinates input only. 
\textbf{\textit{Social LSTM}}~\cite{alahi2016social}: We train the social LSTM model to directly predict trajectory coordinates instead of Gaussian parameters. 
\textbf{\textit{Next}}~\cite{liang2019peeking} is the state-of-the-art method for single-future trajectory prediction on the VIRAT/ActEV dataset. We train the Next model without the activity labels for fair comparison using the code from~\cite{liang2019peeking} {\footnotesize (\url{https://github.com/google/next-prediction/})}. 
%Different from the paper, we train Next model without activity labels for a fair comparison.
\textbf{\textit{Social GAN}}~\cite{gupta2018social} is a recent multi-future trajectory prediction model. We train two model variants (PV \& V) detailed in the paper using the code from~\cite{gupta2018social} {\footnotesize (\url{https://github.com/agrimgupta92/sgan/})}.

\noindent\textbf{Implementation Details.}
We use ConvLSTM~\cite{xingjian2015convolutional} cell for both the encoder and decoder. 
The embedding size $d_e$ is set to 32, and the hidden sizes $d$ for the encoder and decoder are both 256. 
The scene semantic segmentation features are extracted from the deeplab model~\cite{chen2017deeplab}, pretrained on the ADE-20k~\cite{zhou2017scene} dataset.
%The scene semantic segmentation features are resized to (64, 36) and the scene convolution layers are set to have a kernel size of 3, a stride of 2 and the channel dimension is 64. We resize all videos to 1920x1080 and utilize two grid scales, 32x18 and 16x9. The activation function is $tanh$ if not stated otherwise and we do not use any normalization. 
The VIRAT/ActEV official training set as described in the next section for training.
We use Adadelta optimizer~\cite{zeiler2012adadelta} with an initial learning rate of 0.3 and weight decay of 0.001. 
%For Social LSTM, the neighbor is set to 256 pixels as in~\cite{yagi2018future}. 
Other hyper-parameters for the baselines are the same to the ones in ~\cite{gupta2018social}.
We evaluate the top $K=20$ predictions for multi-future trajectories. For the models that only output a single trajectory, including Linear, LSTM, Social-LSTM, and Next, we duplicate the output for $K$ times before evaluating. For Social-GAN, we use $K$ different random noise inputs to get the predictions. For our model, we use diversity beam search~\cite{li2016simple,plotz2018neural} as described in Section~\ref{sec:approach}.


\noindent\textbf{Quantitative Results.} 
Table~\ref{exp-multi} lists the multi-future evaluation results, where we divide the distance-based evaluation according to the viewing angle of camera, 45-degree vs. top-down view. 
We repeat all experiments except \textit{linear} 5 times with random initialization to produce the mean and standard deviation values.
As we see, our model outperforms baselines in all metrics and it performs significantly better on the minADE metric, which suggests better prediction quality over all time instants.
Our model outperforms Social GAN by a large margin of at least 5 points on top-down view, which shows that our method can be benefited from no visual obfuscation in the scene semantic inputs.

\noindent\textbf{Qualitative analysis.} 
We visualize the output of the top 4 methods in Fig.~\ref{f4} from Row 1 and 2. Ours is in Column 4.
% note for the graph
In each graph the yellow trajectories are the observable sequences of each controlled agent and the green trajectories are the ground truth future trajectories. 
The predicted trajectories are shown in yellow heatmaps for multi-future prediction methods and in red lines for single-future prediction methods. 
As we see, our model outputs multiple future paths that match most of the ground truth future trajectories.

\begin{figure}[!t]
	\centering
		\includegraphics[width=0.47\textwidth]{figures/error_analysis.png}
	\caption{Error analysis. See Section~\ref{sec:exp}.}  
	\label{fig:error_analysis}
\end{figure}

\noindent\textbf{Error analysis.}
We show 4 typical errors our model makes in Fig.~\ref{f4} Row 3. The first image shows our model misses the correct direction and the second image shows our model predicts the person will ``go through'' the car instead of go around it. It may be addressed by adding more training examples of ``going around'' car or heuristics of physical constraints.
Our model predicts the person will go to a moving car in the third image, which is due to the lack of modeling of the dynamics of other far-away agents in the scene. 
The four image shows a hard case where the person just exists the vehicle and there is no indication of where they will go next. We leave these solutions to future work.


	
\begin{table}[]
\centering
\small
\begin{tabular}{l||c||c}
\hline
Method & Trained on Real.   & Trained on Sim.        \\ \hline \hline
Linear &  32.19 / 60.92 & 48.65 / 90.84 \\ 
LSTM                &  23.98 / 44.97 & 28.45 / 53.01 \\ 
Alahi \etal~\cite{alahi2016social}         &  23.10 / 44.27 & 26.72 / 51.26 \\ 
Gupta \etal~\cite{gupta2018social}(V)         &  30.40 / 61.93 & 36.74 / 73.22 \\ 
Gupta \etal~\cite{gupta2018social}(PV)         &  30.42 / 60.70 & 36.48 / 72.72 \\ 
Liang \etal~\cite{liang2019peeking}   & 19.78 / 42.43 & 27.38 / 62.11 \\ 
 Ours & \textbf{18.51} / \textbf{35.84} & \textbf{22.94} / \textbf{43.35} \\ \hline
\end{tabular}
\caption{Comparison of different methods on the VIRAT/ActEV dataset. ``rADE/rFDE'' is for models trained on real video training set and ``sADE/sFDE'' is for models trained on the simulation ``anchor'' dataset.} %described in Secion~\ref{sec:dataset}.}
\label{exp-single}
\end{table}

\subsection{Single-Future Prediction on VIRAT/ActEV}\label{sec:exp-virat}
% TODO(junwei): change wording
\noindent\textbf{Dataset \& Setups.} VIRAT/ActEV~\cite{2018trecvidawad} is a public dataset released by NIST in 2018 for activity detection research in streaming video ({\footnotesize \url{https://actev.nist.gov/}}). 
This dataset is a new version of the VIRAT~\cite{oh2011large} dataset, with more videos and annotations. The length of videos with publicly available annotations is about 4.5 hours.
%It includes 455 videos at 30 fps from 12 scenes, more than 12 hours of recordings. Most of the videos have a high resolution of 1920x1080. 
Following~\cite{liang2019peeking}, we use the official training set for training and the official validation set for testing. Other setups are the same as in Section~\ref{sec:exp-multi}.
We use the single-future evaluation metric described in previous section and all the baseline methods as in the multi-future experiments.

\noindent\textbf{Implementation Details.}
We use single-future evaluation metric for this dataset. Each baseline model is allowed one most likely trajectory prediction.
We use the same training setting as previous section.

\noindent\textbf{Quantitative Results.} 
Table~\ref{exp-single} lists the evaluation results in Column 2 and 3. 
As we see, our model achieves state-of-the-art performance and it is especially better on Final Displacement Error (rFDE) metric, thanks to the classification module that helps regulate the model prediction for long-term prediction.
Note that our same model (trained on the same data) achieves best performance on two drastically different tasks (one encourages most-likely single prediction and the other encourages diversity).
The results have validated the efficacy and flexibility of our model.



\begin{table}
\centering
\small
\begin{tabular}{l||c|c}
\hline
Method                             & Single-Future & Multi-Future \\ \hline
Our full model      &   18.54 / 35.95  &    167.2 / 331.8    \\ \hline
No scene graph           &   28.68 / 49.87  & 184.5 / 363.2     \\ 
No regression                 &   53.62 / 83.57   &  232.1 / 468.6 \\ 
No multi-scale training                        &  21.09 / 38.45     &    171.0 / 344.4     \\ \hline
\end{tabular}
\caption{Ablation experiments.}\label{exp-ablation}
\end{table}


\subsection{Ablation Experiments} \label{sec:ablation}
In Table~\ref{exp-ablation} and the last two column of Table~\ref{exp-single}, we evaluate our method through a series of ablation experiments, where for the ``single-future'' column we show the ADE and FDE metrics and for the ``multi-future'' column we show the minADE\textsubscript{20} and minFDE\textsubscript{20} metrics.

\noindent\textbf{Generalizing from simulation to real-world.} As described in Section~\ref{sec:dataset}, we generate simulation data first by reconstructing from real-world videos.
To verify the quality of the reconstructed data and the efficacy of learning from simulation videos, we train models on the simulation videos and evaluate on the test set of VIRAT/ActEV. We have excluded the simulation videos that are reconstructed from the test video of VIRAT/ActEV.
As we see, our model.
The Next~\cite{liang2019peeking} model suffers (a drop of performance from 19.78 to 27.38) from the domain change as it uses low-level visual features which may be pruned to over-fitting.

\noindent\textbf{Effect of using scene graph.} We train our model without scene graph and attention.

\noindent\textbf{Efficacy of two-stage framework.} We test our model without the regression stage and only use the grid center as the coordinate output.

\noindent\textbf{Impact of multi-scale training.} W train our model with single-scale loss.


\begin{comment}
\begin{figure*}[!t]
	\subfigure{\label{fig:ourmodela}}
    \subfigure{\label{fig:ourmodelb}}
    \subfigure{\label{fig:ourmodelc}}
    \subfigure{\label{fig:ourmodeld}}
	\centering
		%\includegraphics[width=1.0\textwidth]{figures/qualitative.pdf}
		\includegraphics[width=1.0\textwidth]{figures/qualitative.png}
		\vspace{-6mm}
	\caption{(Better viewed in color.) Qualitative analysis of our model. Please refer to Fig.~\ref{fig:qualitative-compare} for legends.}  
	\label{fig:qualitative}
	\vspace{-3mm}
\end{figure*}
\end{comment}


==> introduction.tex <==
\section{Introduction}
% intro to the problem
Deciphering humans' future behaviors is a fundamental problem in video understanding. In particular, future path prediction, which aims at forecasting a pedestrian's future trajectory in the next few seconds, has been receiving much attention in our community~\cite{kitani2012activity,alahi2016social,gupta2018social,li2019way}. This functionality proves to be a cornerstone in a variety of applications such as autonomous driving~\cite{bansal2018chauffeurnet,chai2019multipath}, long-term object tracking~\cite{kalman1960new, sadeghian2017tracking}, safety monitoring~\cite{liang2019peeking}, robotic planning~\cite{rhinehart2017first,rhinehart2018r2p2}, socially-aware robots~\cite{luber2010people}, \etc.


% title image: one real world multi-future visualization and one from simulation
\begin{figure}[ht]
	\centering
		\includegraphics[width=0.47\textwidth]{figures/fig1.png} 
	\caption{Our goal is to predict a person's future trajectory with multiple hypothesis. Top-right image shows a person walking in a parking lot from a real video, where the arrow is the actual future trajectory  and the red puddle is the actual future destination of the person. The dashed lines are plausible future trajectories of the person given the observations. Top-left and bottom-right images show our Forking Paths dataset at different viewing angles, where multiple future trajectories and destinations annotated by humans are visualized. Bottom-left image shows the pixel-accurate scene semantic segmentation ground truth.}
	\label{f1}
\end{figure}

% intro to multi-future prediction
The future is nothing but uncertain. Everything remains in a superposition inside the multiverse until it is observed by the external world. Given the exact same historical trajectory, a person is highly likely to take different paths depend on their purpose,  surrounding, or even mood. 
%For example, \lu{use fig 1 to explain this example} a person walking into a parking lot may go to any car or simply pass through them based on , \etc. Therefore, 
An ideal model would not only generate multiple future trajectories but also estimate their probabilities. This problem is known as \emph{multi-future trajectory prediction}~\cite{tang2019multiple,chai2019multipath,li2019way,makansi2019overcoming, thiede2019analyzing,lee2017desire}.
%Predicting the probabilistic future outcomes is crucial for self-driving systems to make safe decisions~\cite{tang2019multiple,chai2019multipath} and in robotic applications to better interpret user intentions.

There are two challenges in the multi-future trajectory prediction. 
(1) How to model the probabilistic distribution of multiple futures? 
(2) How to evaluate the multiple futures in our world where only one outcome can be observed. A few works have been proposed to address the former question using generative models~\cite{gupta2018social,zhao2019multi, sadeghian2018sophie} and mixture density networks~\cite{makansi2019overcoming, thiede2019analyzing, chai2019multipath}. 
%\lu{what's the biggest difference to ours (non-probabilistic outputs? worse transfer?): 
These works used random input vectors to produce multiple future paths and did not explicitly model the probabilistic future.
%did not explicitly model the probabilistic future. For example, Gupta \etal used  to produce multiple future paths. 
For the second challenge, the literature has not yet addressed due to the impossibility of observing multiple futures in the real world videos. The existing evaluation is hence only performed against a single deterministic future trajectory in the common benchmark.

In this paper, we propose a model to estimate the probabilistic future trajectories. Different from prior works~\cite{gupta2018social,zhao2019multi}, we explicitly model the problem as a Markov chain over a spatial graph of scene segmentation and learn the probabilistic future by a graph neural network. We introduce two important techniques for more accurate estimation.
First, our model represents a video scene as a \emph{spatial scene graph} with the node indicating the semantic segmentation feature of a spatial region (\eg cars on the road, persons on the sidewalk) and edges as the spatial adjacency between two regions. The graph is modeled by the graph attention network over the semantic segmentation features. This symbolic abstraction significantly improve the model's generalization performance. 
Second, our model predicts multiple futures using a dual-head, including a classification head predicting the probability of entering a spatial region and a regression head compensating the offset to the true destination in the pixel space. 
%Using dynamic programming, we can compute the probability for any sequence of time steps (\ie the probabilistic distribution of future paths).

% Mulit-future dataset
We also discuss a feasible plan to evaluate multi-future path prediction in 3D simulation. To be specific, we establish a simulation dataset in CARLA~\cite{dosovitskiy2017carla} where human annotators are asked to take control of the agent to navigate in the simulation scenes reconstructed from the real-world video. 
Given the same observation (See Fig.~\ref{f1}), different annotators control the same agent and produce multiple trajectories.
As shown in the top-left and bottom-right of Fig.~\ref{f1}, we overlay multiple future trajectories produced by different annotators.
%the person walking in the parking lot could be going to one of the cars or simply continue walk through the parking.
%While in the top-right image from real videos the person's actually future trajectory is the thicker arrowed line, our dataset recreates this moment and plausible multi-future trajectories are collected for evaluation.
%In this way, multiple future paths can be approximately observed through the control sequence of the real humans. 
We compute distance-based metrics to quantitatively evaluate the predicted multiple future trajectories. We use the simulation in our study for several unique benefits. 
First, it ensures the identical observable history to be shared among different humans. This is impossible in real world since no man ever steps in the same river twice. 
Second, the simulation provides pixel-accurate ``free labels'' such as the pedestrians' paths, bounding boxes, and scene semantics for the entire video from different camera angles. The top-left and bottom-right of Fig.~\ref{f1} shows two views of the same scene. 
Finally, our experiments show that models trained on simulation data generalizes reasonably well on real-world videos, and vice versa, indicating a small domain discrepancy between our simulation data and the real world data.


% simple intro of the collection process
%We ask human annotators to control agents in reconstructed scenes from real-world videos to navigate to predefined destinations.
% benefits
%The benefits of our dataset are two folds:
%First, for each multi-future trajectory sequence, we control the observation conditions to be exactly the same so that models can be judged fairly.
%Second, we use real human annotators to perform a possible future course of actions given the same observations.


We empirically validate our model on the challenging real-world benchmark ActEV/VIRAT~\cite{oh2011large,2018trecvidawad} for single-future trajectory prediction, in which our model achieves the best published result. On the proposed simulation data for multi-future prediction, experimental results show our model performs favorably against the state-of-the-art models across different settings. To summarize, the contributions of this paper are threefold:
\textit{(i)} We introduce a feasible evaluation plan, along with a benchmark, for multi-future path prediction. It is the first multi-future trajectory benchmark created by real humans.
\textit{(ii)} We propose a new effective two-stage framework to explicitly tackle the problem of multi-future trajectory prediction. Our model can be generalized by using scene semantic segmentation and graph attention network.
\textit{(iii)} Our model achieves the best-published result on the challenging ActEV/VIRAT benchmark. Ablation studies are conducted to verify that our model can be generalized from simulation to real-world scenes.





%Even if one may generate multiple outcomes, in reality, it is nearly impossible to accesses multi-future trajectories with the same observation. As a result, the evaluation remains to be a challenging issue in the literature.
%path prediction requires an understanding of the static scene and the dynamics of the moving objects. A model will need to take into account the fact that people navigate through public spaces differently and with latent goals in mind.
%We will not be able to know exactly what a person will do next due to the inherent complexity of human decisions. 
% why multi future is important
%It is important for a model to predict multiple outcomes and their possibilities to help self-driving system make safe decisions.
%Previous works have tried to predict the stochastic multi-future implicitly using generative models~\cite{gupta2018social,zhao2019multi} with random vector inputs to assimilate various factors that affect human decisions.
% what we propose
% How we solve the two challenges

% First, since People navigate in public spaces differently by taking into account the dynamics of the scene, our model describes the dynamic scene as spatial scene graphs with semantic nodes like cars and sidewalk.
% Second, we propose a simple yet effective framework that utilizes a two-stage prediction process that mimics the process of human decisions. Intuitively, human decides where they want to go and makes small decisions of how to navigate along the way by considering neighbouring scene dynamics. 
% Our model first predicts which node the person is going to go at each future time-instant. 
% Then the model predicts the offsets from each node's spatial center to the exact future locations, which produces a fine-grained prediction from the coarse scene graph nodes.
% \lu{put this to related work: Our work borrows this idea from the proven two-stage framework~\cite{ren2015faster} in object detection.}
% % benefit of our method
% Our framework is flexible and able to generalize to different scenes and dynamic situations.

==> kevin/beam-search_kevin.tex <==
To generate multiple qualitatively distinct
 trajectories, we use the diverse beam search strategy from \cite{li2016simple}.
 To define this precisely,
 let $C_t=f_C(H_t^C)$ be the classification decoder
 in \cref{eqn:fC},
 and $H_t^C=f_H(H_{t-1}^C,A_{t-1})$ be the RNN update
 in \cref{eqn:fH}.
 Here we use a single index $i \in [1, H \times W]$ to represent grid cells.
 Define
 \begin{align}
C_{t|i} = f_C(f_H(H_{t-1}^C, A_{t-1}=i))
\end{align}
as the distribution over grid cells at time $t$ given that we
%were previously in cell $i$.
previously selected cell $i$.
Define
\begin{align}
    S(i) = \argmax_j C_{t|i}(j) + \gamma(i,j)
\end{align}
as the top $K$ successor to cell $i$,
where $\gamma(i,j)$ is a diversity term that encourages
the selection of cells that are not too close and $C_{t|i}(j)$ represents the probability of selecting cell $j$.
Let $M_{t-1}$ be a list of the top $K$ cells in the previous step.
We compute the new beam using
\begin{align*}
    M_t = [S(M_{t-1,1}), \ldots, S(M_{t-1,K})]
\end{align*}
If $K=1$, this reduces to greedy search
(and $M_t=A_t$).

Once we have computed the top $K$ grid cells per time step,
we add the corresponding offset vectors to produce
$K$ predicted locations $L_{t,k} \in \real^2$.
This constitutes the final output of our model.

==> methods1.tex <==



\section{Multi-Future Prediction Model}
\label{sec:approach}

\begin{figure*}[!t]
	\centering
		\includegraphics[width=1.0\textwidth]{figures/cvpr2020_model.png}
	\caption{Overview of our model. Our model takes abstract scene semantic segmentation as input and utilizes a Spatial-Temporal Feature Encoder to extract historic information. Then we use a graph attention decoder along with a dual-head output module to get multi-future trajectory prediction.}  
	\label{f2}
\end{figure*}

\begin{comment}
\begin{figure}[t]
	\centering
		\includegraphics[width=0.47\textwidth]{figures/grid_loss.png}
	\caption{Activity location prediction with classification and regression on the multi-scale Manhattan Grid. See Section~\ref{sec:cls_rg}.}
	\label{grid_loss}
	\vspace{-5mm}
\end{figure}
\end{comment}


Our goal is to learn a model that can forecast an agent's multiple future trajectories from a given training set in different environments with each environment represented as a set of discrete spatial landmarks. At test time, given an agent's observable trajectory in an seen or unseen environment, the model produces a distribution of future trajectories in the environment. 

\subsection{Problem Formulation}
Formally, let ${s}_i(1 \timeto t)$ and ${a}_i(1 \timeto t)$ be the set of observable states and actions from time 1 to $T$ for the $i$-th trajectory. We partition a calibrated video scene in Euclidean space into a graph over a $H$x$W$ grid. %consider the landmark/state to be the grid in the graph. See Fig.~\ref{}. 
Our goal is to learn a model to predict:
\[
P(s_i(t \!+ \!1 \timeto t\!+\!T), a_i(t\!+\!1 \timeto t\!+\!T) | s_i(1 \timeto t), {a}_i(1 \timeto t), G, \mathcal{D})
\]
where $\mathcal{D}$ is set of training trajectories. $G$ is named \emph{spatial scene graph} where each node is a region in the grid (state) and an edge exists between neighboring states in space to capture the prior knowledge that people cannot teleport. ${s}_i(1 \timeto t)$ is the sequence of observed states visited in $G$ so far and ${s}_i(t \!+ \!1 \timeto t\!+\!T)$ is the forecasted trajectory. Likewise, ${a}_i(1 \timeto t)$ and ${a}_i(t\!+\!1 \timeto t\!+\!T)$ are the sequences of observed and forecasted actions. For notational simplicity, we will combine ${s}$ and ${a}$ into a single tenor ${x}$.

Let $S=f({x} (1 \timeto t), G, \mathcal{D})$ be a function of all observed information for a sequence. $S$ is a sufficient statistic for forecasting the future trajectories. Hence we use a first order discrete Markov model:
\begin{equation}
P({x}(t+1 \timeto t+T) | {x}(1 \timeto t), G, \mathcal{D}) = \prod_{h=t+1}^{t+T} P({x}(h) | {x}(h-1), S),
\end{equation}
where $\mathbf{A}_{ij} = P({x}(h)=j | {x}(h-1)=i, S)$ is the transition matrix for the test sequence over the discrete states. According to the Chapman-Kolmogorov theorem, we can generate the state distribution $T$ steps into the future by iteratively computing $\pi (t+1) = \mathbf{A}^\intercal \pi (t)$, where $\pi(t)$ is the state distribution for the time $t$.

Our problem has a key difference to the standard Markov model: the meaning of the discrete states differs from sequence to sequence and time to time depending on the underlying graph representation $G$. Hence, we parameterize the transition matrix by a neural network:
\begin{equation}
\label{eq:Ai}
\mathbf{A}_{i:} =\text{softmax} (g(\phi(v_i), \phi(\mathcal{N}_{i}); \Theta)),
\end{equation}
where $g$ is the graph neural network over the node $v_i$ and its spatially adjacent neighbors $\mathcal{N}_{i}$. $\phi$ is a module to encode the spatial-temporal feature for the node and edge in $G$.



\subsection{Network Architecture}
We propose a network called \emph{\fancyname} to compute the state distribution $\pi(t)$. Fig.~\ref{f2} shows its overall architecture. 
It has three key components. The spatial-temporal feature encoder extracts the scene semantics for a trajectory. In the Graph Attention Decoder module, we compute the transition matrix in Eq.~\eqref{eq:Ai} and the state distribution. Finally, Dual Prediction Head calculates the state distribution over all regions in the grid (classification) and estimates offsets between the destination and the grid center. We will discuss each module in details below.
% \noindent\textbf{Spatial-Temporal Encoder} extracts abstract scene semantic information along the person's path.
% \noindent\textbf{Graph Attention Decoder} looks at the interaction between each node in the scene and their surroundings to determine the likelihood of the person traveling to a location.

%--------------------------------------------------------------------
\subsubsection{Spatial-Temporal Feature Encoder}
This module encodes an agent's observable trajectory from time 1 to $t$ by dynamic scene semantics. Specifically, we divide a video scene in Euclidean space into a discrete $H \times W$ grid. A trajectory is represented by a sequence of one-hot vectors over the grid: $\mathbf{P} \in \mathbb{R}^{t \times H \times W \times 1}$. Since the agent can only be in one place at a time, we set the dimension of the corresponding region in $\mathbf{P}_t$ to 1, and 0 otherwise. Inspired by~\cite{lazebnik2006beyond,lin2017feature}, we train our network with different grid scales and show its benefits in Section~\ref{sec:ablation}. For convenience, our discussion will be on the single $H \times W$ grid.

We extract the scene semantic segmentation from time 1 to $t$ using a pretrained model from the ADE20k~\cite{zhou2017scene} dataset. The pixel-level label is resized down to $H \times W$ using nearest neighbour interpolation and encoded into $\mathbf{S} \in \mathbb{R}^{t \times H \times W \times (N_{s}+1)}$ by the one-hot encoding, where $N_{s}$ is the number of unique scene classes. We append an additional class to model the background. Our model uses only the high-level scene semantic features as opposed to RGB pixel features in most existing works for a reason. That is to generalize better to novel scenes in real-world videos and, furthermore, to generalize between the real and simulation video.

To obtain the spatial-temporal feature shown in Fig.~\ref{f2}, we have:
\begin{equation}
\mathbf{X}_k = \text{convRNN}(\mathbf{P}_k \odot (\mathbf{W}_{k} * \mathbf{S}_k), \mathbf{X}_{k-1}), \forall k \in [1,t]
\end{equation}
where $d_{enc}$ is the hidden state dimension of the convolutional RNN~\cite{xingjian2015convolutional,wang2019eidetic}. $\odot$ is element wise product, and $*$ represents 2d-convolution. The last hidden state $\mathbf{X}_{t} \in \mathbb{R}^{H \times W \times d_{enc}}$ summarizes the entire surrounding scenes and will be used as our spatial-temporal feature.

% and we show the benefits in the experiment Section~\ref{sec:ablation}.
% Then we use $P_{obs}$ to mask out locations where the person is not in and apply convolutional recurrent neural network (convRNN)~\cite{xingjian2015convolutional} to encode the temporal information at each location. 



% use the last hidden state $\mathbf{X}$
% Intuitively, the encoded features $\mathbf{X}$ at time $T_{obs}$ represents the history of the person's path. At each location that the person has ever traveled, $\mathbf{X}$ encodes the its past including what the surrounding scenes are from where the person has moved to.
% We use the last time instant of the hidden state for $\mathbf{X}_{:,t}$ the following modules.

% First, learning from semantic classes makes generalizing to novel scenes easier.
% Second, since we utilize 3D simulation data as described in Section~\ref{sec:dataset} and there is a realistic gap between RGB simulation and real-world, our model trained on semantic data can perform better on real-world videos as shown in Section~\ref{sec:ablation}.
% As we see, it adopts abstract scene semantics in most of the existing works. Our results show this simple abstraction improves generalization to novel scenarios and environments.
%Then we encode the spatial-temporal feature. convolutional operations with strides to get features of different scales.



%$\mathcal{N}_{v_j}$ is a set of n in the spatial graph $G$ and $\phi$  the feature of $v_i$. The final function $g$ is parameterized by $\Theta$. In this paper
\subsubsection{Graph Attention Decoder}
This module decodes the spatial-temporal feature extracted in the previous module. We represent a video scene by the \emph{spatial scene graph} where a node is a spatial region in the grid and is connected to its only 8 neighboring nodes. An edge hence represents a legit transition between two nodes at any time instance. We use the graph attention network~\cite{velivckovic2017graph} to represent the features in our model:
\begin{equation}
\begin{split}
    \phi(v_i) &= [\mathbf{h}_{i:};\mathbf{\bar{S}}]\\
    \phi(\mathcal{N}_i) &= \mathbf{\tilde{h}}_{i:} = \frac{1}{|\mathcal{N}_i|} \sum_{v_j \in \mathcal{N}_i} f_{edge}(v_i, v_j) \cdot \mathbf{h}_{j:} + \mathbf{h}_{i:}
\end{split}\label{eq:nodefeature},
\end{equation}
where $\mathbf{h} \in \mathbb{R}^{HW \times d_{dec}}$ is the hidden state of the RNN decoder.   $\mathbf{h}_{i:} \in \mathbb{R}^{d_{dec}}$ indicates the node feature for the $i$-th region in the graph. $\mathbf{\bar{S}} = \frac{1}{t} \sum_{k=1}^t \mathbf{S}_{k:}$ is the average pooling of $\mathbf{\bar{S}}$ over the temporal dimension and $[\cdot;\cdot]$ is the concatenation operation. $f_{edge}(\cdot)$ is an attention function to compute edge weight between node $v_i$ and node $v_j$. For simplicity, we use a fully-connected layer with softmax to compute the attention.

%Graph attention network~\cite{velivckovic2017graph} has been used for future prediction~\cite{sun2019relational} due to its ability to model important relations.
% where . $\mathcal{N}_i$ denotes the neighbors of node $i$. In this paper we only consider direct neighbors hence the number of neighbors is 8 for each node.
% Following ~\cite{sun2019relational}, $f_{edge}(\cdot)$ is implemented using an attention function.
% In this paper, we use simple matrix multiplication with a softmax function for attention computation.

We use the convRNN~\cite{xingjian2015convolutional} as our decoder for recurrent prediction:
\begin{equation}
\begin{split}
    \mathbf{h}_k &= \text{convRNN}(\mathbf{\tilde{h}}_{k-1}), \forall k \in [1,t] \\
    \tilde{\mathbf{h}}_k &= [\phi(\mathcal{N}_1); \cdots; \phi(\mathcal{N}_{H\times W})].
\end{split}\label{eq:decoder}
\end{equation}
Here we overload the notation and use the subscript to index time. $\mathbf{h}_0$ is initialized as our encoder output $\mathbf{X}_{t}$. The feature $\phi(\mathcal{N}_i)$ is from Eq.~\eqref{eq:nodefeature}. $\tilde{\mathbf{h}}_k$ and $\mathbf{h}_k$ have the same shape $HW \times d_{dec}$ but $\tilde{\mathbf{h}}_k$ contain the encoded trajectory in the spatial scene graph.



%The node feature is represented as $\mathbf{v}^t = [\mathbf{h}^{t};\mathbf{\bar{S}}]$
%We treat each location as a node and the node feature is represented by: , where $\mathbf{S}'_e$ is the encoded scene semantic features averaged across the temporal dimension and $[\cdot;\cdot]$ is the concatenation operation along the last dimension.
%and its numerical value equals the transition probability.

%We utilize convRNN~\cite{xingjian2015convolutional} for recurrent prediction.
%To initialize the prediction, we use the last hidden states from the spatial-temporal encoder $\mathbf{X}' \in \mathbb{R}^{H \times W \times d}$ and the last observation of the person's path $\mathbf{P}'_{obs}$.
%Each spatial location in become nodes in the graph. Each node is only connected to their neighbouring 8 nodes and itself. 
%The node features are represented in the hidden states of the recurrent operation and the encoded scene semantic segmentation features at the location. 
% See Fig.~\ref{f2} ``Graph Attention Decoder'' for a sketch of the module.


% TODO(junwei): change wording of this 
% Our current model captures the dynamic location predictions without scene semantics around each location. As shown in previous works~\cite{kitani2012activity,sadeghian2018sophie}, scene semantic information is important for future path prediction. Motivated by recent success in relational reasoning, we combine graph neural network (GNN) with convolutional recurrent models. 

%More complex attention mechanism like self-attention~\cite{vaswani2017attention} and focal attention~\cite{liang2018focal,liang2019focal} can be utilized to better model the relations between nodes. We leave this exploration to future work.
% We utilize a residual link to get the new hidden state as this technique has shown to be effective in many applications~\cite{he2016deep,girshick2015fast}. The new hidden state is then used in the convRNN update function for the next time-instant.

%TODO(junwei): change wording
\subsubsection{Classification \& Regression Module} \label{sec:cls_rg}
We propose to use two heads for trajectory prediction: a classification head to predict which grid the agent is going and a regression head to estimate the exact location inside the grid block. The classification prediction at time $t$ is given by:
\begin{equation}
\mathbf{O}_t = \text{softmax}(W_{l} * \mathbf{h}_t) \in  \mathbb{R}^{H \times W}.
\end{equation}
$\mathbf{O}_t$ is an approximation of the state distribution $\pi(t)$ and concatenating $\mathbf{O}_t$ over the time yield the final classification output $\mathbf{O}^{cls} \in \mathbb{R}^{t \times H \times W}$.

Since the classification prediction is on the coarse grid, to refine the prediction, the regression head predicts the deviation of each grid block center to the true location $x$-$y$ coordinates in pixel space. We utilize a separate graph attention decoder for regression and denote its output as $\mathbf{O}^{reg} \in \mathbb{R}^{t \times H \times W \times 2}$.
The final trajectory output at time $t$ can be written as:
\begin{equation}
\label{eq:output}
\mathbf{Y} = (\mathbf{C} + \mathbf{O}^{reg}) \odot \argmax \mathbf{O}^{cls},
\end{equation}
where $\mathbf{C}$ is the $x$-$y$ coordinates of each grid center, and $\argmax$ operation is applied to the spatial dimension.



Our idea is partially inspired by RPN~\cite{ren2015faster} in object detection. Different from prior works~\cite{bansal2018chauffeurnet,li2019way,manh2018scene,xue2018ss,liang2019peeking}, our model introduces an additional regression network for sequential fine-grained prediction. It is worth noting that a very recent work~\cite{chai2019multipath} also designed a two-stage prediction, where their classification targets are pre-defined anchor trajectories. Our method differs in that it can learn to predict arbitrary trajectories, not limited by the number of predefined anchors.

Our two-stage framework has the following benefits:
(i) it provides more accurate results using a coarse-to-fine prediction paradigm, which has shown to be effective in many works~\cite{lin2017feature,chen2017rethinking}; 
(ii) it models the state distribution enabling multi-future trajectory prediction while still taking advantages of more accurate models that directly output $x$-$y$ coordinates.

% and recent works have also adopted similar ideas~\cite{chai2019multipath, liang2019peeking,manh2018scene,bansal2018chauffeurnet,li2019way,xue2018ss}.
% Different from , . Unlike ~\cite{liang2019peeking}, we utilize temporal modeling for sequential prediction instead of only single location prediction. 
% First, the model predicts a coarse location where the person might be going and then a second regression model predicts the exact future locations in terms of offset from the center of the coarse location.
% Formally, the video frame is divided into a rectangle grid of size $H \times W$. Given the output from the graph attention decoder $\mathbf{h} \in \mathbb{R}^{T_{pred} \times H \times W \times d}$, the classification output at time $t$ is given by
% $f_{out}(\cdot)$ is the output function which will be discussed in Section~\ref{sec:cls_rg}.


% Then we convert $\mathbf{l}'^t$ to a one-hot vector after applying $\argmax$ and we get  $\mathbf{l}^t$ in Equ.~\ref{eq:convrnn}.
% The final classification output is $\mathbf{l}_{cls} \in \mathbb{R}^{T_{pred} \times H \times W}$.
% discuss related work here
% TODO(junwei): change wording

\subsection{Training and Inference}
% Following the settings of previous works~\cite{alahi2016social,gupta2018social,sadeghian2018sophie,liang2019peeking}, we assume each scene is first processed to obtain the spatial coordinates of the target persons during the observation period. 
Our model trains on the observed trajectory from time 1 to $t$ and predicts the future trajectories (in the $xy$-coordinates) from time $t+1$ to $t+T$. For classification, the cross-entropy loss is used:
\begin{equation}
    L_{cls} = -\frac{1}{T} \sum_{k=t+1}^{t+T} \sum_{i=1}^{H} \sum_{j=1}^W \mathbf{P}_{kij} \log(\mathbf{O}^{cls}_{kij})
\end{equation}
For regression, we use the smoothed $L_1$ loss in object detection~\cite{ren2015faster}:
\begin{equation}
 L_{reg} = \frac{1}{T} \sum_{k=t}^{t+T} \text{smooth}_{L_1}(\mathbf{O}^{reg}_k, \mathbf{I}_k)
\end{equation}
where $\mathbf{I}_k$ is the ground truth difference to the correct grid block center at time $k$. 

The final loss is then calculated from $L = L_{cls} + \lambda L_{reg} + \|\Theta\|$, where $\|\Theta\|$ is the weight decay term. We use a balance controller $\lambda = 0.1$ for regression to compensate its higher loss values during training.

For inference, our model outputs a distribution over all states at each time instant in a recurrent fashion. The likelihood of a trajectory will change if the agent executes different actions. Eq.~\eqref{eq:output} shows a single-future trajectory prediction by greedy search. To get multiple trajectories, we use the diverse beam search strategy in~\cite{li2016simple} to get the top $N$ best trajectories with diversity. Suppose $K$ denotes the beam size and let $Y^{k}_{t-1}=\{y^k_1, \dots, y^k_{t-1}\}, k \in [1, K]$
\lu{not finished}

$b$ hypotheses at time $t-1$ are denoted as, the probabilities for each new $K \times K$ hypothesis is computed as follows:
\begin{equation}
\begin{split}
    &P(Y^{k}_{t-1}, y^{k,k'}_t \,|\, \mathbf{O}^{cls}_{t-1} ) \\
    &= P(Y^{k}_{t-1} \,|\, \mathbf{h}^{t-1} ) + \log p(y^{k,k'}_t \,|\, \mathbf{l}^{t-1}_{cls}, Y^{k}_{t-1}) + \gamma k'
\end{split}
\end{equation}
where $y^{k,k'}_t$ means selecting $k'$ at time $t$ for previous hypothesis $k$ and $\gamma$ is a diversity term.
%\lu{training consider all pixel offset to all boxes for now.}



% it will have different outputs if we select different locations as next inputs. In Equ.~\ref{eq:output} we use a greedy search strategy. 
% Inspired by works in language modeling and neural generation~\cite{bengio2003neural,li2016simple}, we utilize a diverse beam search strategy similar to ~\cite{li2016simple} to get diverse N-best trajectory predictions.
% Formally, 

==> related_work.tex <==
\section{Related Work}
Future trajectory prediction models mostly try to predict the future path of pedestrians and vehicles.
% crowd/inter-person 
A large body of work learns to predict person path by considering human social interactions and behaviors in crowded scene~\cite{xu2018encoding,yi2016pedestrian,zou2018understanding,alahi2016social,gupta2018social}.

\noindent\textbf{Single-future trajectory prediction.}
Social-LSTM~\cite{alahi2016social} added social pooling to model nearby pedestrian trajectory patterns. 
Scene-LSTM~\cite{manh2018scene} divided the static scene into Manhattan Grid and predict pedestrian's location using LSTM. 
CAR-Net~\cite{sadeghian2018car} proposed an attention network on top of scene semantic CNN to predict person trajectory.
Some recent works have attempted to predict person path by utilizing individual's visual features instead of considering them as points in the scene. Kooij \etal in~\cite{kooij2014context} looked at pedestrian's faces to model their awareness to predict whether they will cross the road using a Dynamic Bayesian Network in dash-cam videos. Yagi \etal in ~\cite{yagi2018future} used person keypoint features with a convolutional neural network to predict future path in first-person videos. 
Chauffeurnet~\cite{bansal2018chauffeurnet} utilized imitation learning to predict vehicle future trajectories.
Hong \etal~\cite{hong2019rules} utilized semantic inputs to predict driving behavior.
Ma \etal~\cite{ma2017forecasting} used appearance features to forecast pedestrian future trajectories.
SS-LSTM~\cite{xue2018ss} utilized a multi-scale LSTM to predict pedestrian trajectories.
Zhao \etal~\cite{zhao2019multi} proposed a tensor-fusion network to predict vehicle trajectories.
SR-LSTM~\cite{zhang2019sr} added a states refinement module to social-LSTM~\cite{alahi2016social} for better person path prediction.
Recently Liang \etal ~\cite{liang2019peeking} proposed a joint future activity and trajectory prediction framework that utilized multiple visual features.

\noindent\textbf{Multi-future trajectory prediction.}
Social-GAN~\cite{gupta2018social} added adversarial training on Social-LSTM to improve performance. 
A number of works focused on learning the effects of the physical scene, \eg, people tend to walk on the sidewalk instead of grass. 
Kitani \etal in ~\cite{kitani2012activity} used Inverse Reinforcement Learning to forecast human trajectory. 
SoPhie~\cite{sadeghian2018sophie} combined deep neural network features from scene semantic segmentation model and generative adversarial network (GAN) using attention to model person trajectory.
DESIRE~\cite{lee2017desire} utilized variational auto-encoders (VAE) to predict future vehicle trajectories.
Makansi \etal~\cite{makansi2019overcoming} proposed a convolutional neural network to predict multiple mixture of gaussians.
Li \etal~\cite{li2019way} proposed a novel Imitative Decision Learning approach to predict person future paths with multiple possibilities.
Thiede \etal~\cite{thiede2019analyzing} analyzed the variety loss for multi-future vehicle trajectory prediction.
Chai \etal~\cite{chai2019multipath} utilized anchor trajectories and a two-stage framework to predict multiple trajectories for vehicles.
Inverse Reinforcement Learning (IRL)~\cite{rhinehart2018r2p2,rhinehart2019precog} was proposed for conditioned forecasting.

\noindent\textbf{Future Prediction with CNNs.} 
Many works have utilized CNN for future predictions~\cite{wang2018video, wang2019eidetic}.
Luc \etal~\cite{luc2017predicting} utilized Convolutional Neural Network to predict future scene semantic sementation.
VID2VID ~\cite{wang2018video} used generative adversarial networks to predict future video frames.


\noindent\textbf{Trajectory Datasets.}
%\junwei{reduced and merged}
%\lu{Junwei shall we reduce and merge this into the dataset motivation.}
Many vehicle trajectory datasets~\cite{caesar2019nuscenes,chang2019argoverse} have been proposed as self-driving gains a lot of attention in the research community. 
Due to the recent advancement in 3D computer vision research~\cite{zhang2015fast,liang2017event,shah2018airsim,dosovitskiy2017carla,richter2016playing,ros2016synthia,heess2017emergence}, many research works~\cite{qiu2017unrealcv, gaidon2016virtual,de2017procedural,das2018embodied,wu2019revisiting,zhu2017target,sun2019stochastic} have looked into 3D simulated environment for its flexibility and ability to generate enormous amount of data.
%EmbodiedQA~\cite{das2018embodied,wu2019revisiting} utilized a virtual 3D house simulation to learn question answering by exploring the environment.
%Nicolas \etal ~\cite{heess2017emergence} used a 3D physical engine to let agent learn to move from scratch.
%Ritchter \etal ~\cite{richter2016playing} collected photo-realistic data from computer games.
%AI2-THOR dataset ~\cite{zhu2017target} was collected for visual navigation.
%Many works ~\cite{qiu2017unrealcv, gaidon2016virtual,de2017procedural} were proposed to use data generated from 3D simulation for video object detection, tracking and action recognition analysis. 
%Recently Sun \etal ~\cite{sun2019stochastic} proposed a forecasting model by using a gaming simulator.
%AirSim ~\cite{shah2018airsim} and CARLA ~\cite{dosovitskiy2017carla} were proposed for robotic autonomous controls for drones and vehicles.
We are the first to propose a 3D simulation dataset that is reconstructed from real-world scenarios with human annotator behaviors for multi-future person trajectory prediction. More comparison with other datasets is discussed in Section~\ref{sec:dataset}.







